Towards Lingua Franca Named Entity Recognition with BERT

Information extraction is an important task in NLP, enabling the automatic extraction of data for relational database filling. Historically, research and data was produced for English text, followed in subsequent years by datasets in Arabic, Chinese (ACE/OntoNotes), Dutch, Spanish, German (CoNLL evaluations), and many others. The natural tendency has been to treat each language as a different dataset and build optimized models for each. In this paper we investigate a single Named Entity Recognition model, based on a multilingual BERT, that is trained jointly on many languages simultaneously, and is able to decode these languages with better accuracy than models trained only on one language. To improve the initial model, we study the use of regularization strategies such as multitask learning and partial gradient updates. In addition to being a single model that can tackle multiple languages (including code switch), the model could be used to make zero-shot predictions on a new language, even ones for which training data is not available, out of the box. The results show that this model not only performs competitively with monolingual models, but it also achieves state-of-the-art results on the CoNLL02 Dutch and Spanish datasets, OntoNotes Arabic and Chinese datasets. Moreover, it performs reasonably well on unseen languages, achieving state-of-the-art for zero-shot on three CoNLL languages.

==> tables/conll_dev_cased_perf_by_frz_layers.tex <==

\begin{table}
\begin{center}
\begin{tabular}{lrrr}
\toprule
{} &   deu &   esp &   ned \\
frz &       &       &       \\
\midrule
-1  & 76.92 & 74.13 & 80.95 \\
 0  & 76.42 & 73.97 & 79.76 \\
 1  & 77.96 & 74.85 & 80.59 \\
 2  & 78.76 & 74.57 & 81.29 \\
 3  & 78.49 & 73.79 & 81.38 \\
 4  & 78.34 & 73.58 & 80.98 \\
 5  & 78.78 & 72.93 & 80.58 \\
 6  & 77.53 & 72.62 & 80.16 \\
 7  & 76.73 & 72.65 & 80.16 \\
 8  & 74.15 & 70.97 & 79.16 \\
 9  & 67.91 & 70.34 & 77.10 \\
 10 & 58.80 & 64.60 & 72.28 \\
 11 & 59.62 & 63.49 & 73.08 \\
 12 & 43.94 & 53.87 & 54.30 \\
\bottomrule
\end{tabular}

\caption{}
\label{tab:conll_dev_cased_perf_by_frz_layers}
\end{center}
\end{table}


==> tables/conll_exps_cased_dev.tex <==
\begin{table}
\begin{center}
\begin{tabular}{llrrrr}
\toprule
      & lang &   German &   eng &   esp &   ned \\
model & frz &       &       &       &       \\
\midrule
CL & -1  & 76.05 & 78.30 & 73.85 & 83.25 \\
      &  8  & 74.41 & 76.40 & 71.14 & 82.61 \\
CL+LI & -1  & 75.30 & 79.09 & 72.09 & 83.13 \\
      &  8  & 74.85 & 77.87 & 70.68 & 81.66 \\
LI & -1  & 77.95 & 77.54 & 73.74 & 83.23 \\
      &  8  & 78.40 & 78.44 & 72.07 & 81.64 \\
ML & -1  & 77.28 & 77.36 & 75.87 & 82.41 \\
      &  8  & 76.26 & 77.22 & 72.97 & 83.19 \\
PC & -1  & 77.57 & 78.61 & 73.78 & 82.42 \\
      &  8  & 74.92 & 78.61 & 71.91 & 81.75 \\
PC+LI & -1  & 75.59 & 78.60 & 73.03 & 81.15 \\
      &  8  & 73.45 & 78.04 & 72.12 & 81.52 \\
\bottomrule
\end{tabular}
\caption{CONLL dev results using ML, LI, CL, CL+LI and different
  frozen layers.}
\label{tab:conll_exps_cased_dev}
\end{center}
\end{table}


==> tables/conll_exps_cased_tst.tex <==
\begin{table}
\begin{center}
\begin{tabular}{llrrrr}
\toprule
      & lang &   German &   English &   Spanish &   Dutch \\
model & frz &       &       &       &       \\
\midrule
CL & -1  & 69.11 & 74.41 & 75.29 & 82.37 \\
      &  8  & 67.37 & 73.24 & 73.11 & 81.23 \\
CL+LI & -1  & 68.94 & 74.51 & 73.68 & 81.13 \\
      &  8  & 66.93 & 74.50 & 73.85 & 80.56 \\
LI & -1  & 72.35 & 73.87 & 75.61 & 80.97 \\
      &  8  & 72.30 & 74.91 & 73.76 & 80.40 \\
ML & -1  & 70.34 & 73.31 & 77.17 & 80.14 \\
      &  8  & 70.56 & 74.29 & 75.46 & 81.42 \\
PC & -1  & 70.86 & 73.72 & 75.57 & 80.28 \\
      &  8  & 67.47 & 75.68 & 74.84 & 80.09 \\
PC+LI & -1  & 70.11 & 74.79 & 74.51 & 79.53 \\
      &  8  & 65.47 & 74.79 & 74.33 & 80.55 \\
\bottomrule
\end{tabular}
\caption{CONLL test results using ML, LI, CL, CL+LI and different
  frozen layers.}
\label{tab:conll_exps_cased_tst}
\end{center}
\end{table}


==> tables/conll_frz_cased_tst.tex <==
% \begin{table}
% \begin{center}
% \begin{tabular}{lrrrr}
% \toprule
% lang &   deu &   eng &   esp &   ned \\
% frz &       &       &       &       \\
% \midrule
% -1  & 70.34 & 73.31 & 77.17 & 80.14 \\
%  0  & 70.95 & 72.97 & 76.87 & 79.61 \\
%  1  & 70.82 & 73.57 & 76.85 & 82.21 \\
%  2  & 72.66 & 72.94 & 77.06 & 81.94 \\
%  3  & 72.96 & 73.61 & 77.08 & 83.35 \\
%  4  & 72.26 & 73.92 & 76.50 & 82.80 \\
%  5  & 73.61 & 74.04 & 76.45 & 82.76 \\
%  6  & 72.96 & 73.73 & 75.75 & 82.65 \\
%  7  & 71.80 & 76.20 & 75.69 & 82.23 \\
%  8  & 70.56 & 74.29 & 75.46 & 81.42 \\
%  9  & 66.05 & 73.41 & 74.02 & 79.61 \\
%  10 & 62.23 & 72.21 & 72.49 & 78.17 \\
%  11 & 60.38 & 70.06 & 70.83 & 76.63 \\
%  12 & 43.77 & 59.73 & 58.68 & 64.21 \\
% \bottomrule
% \end{tabular}
% \caption{Cased multilingual zero shot on CONLL TEST data. frz
%   corresponds to number of frozen layers during training. -1 is where
%   nothing is frozen and is the standard setting. 0 is where only the
%   embedding is frozen. 1 is embedding and first layer is frozen and so
%   forth. 12 is where all bert layers are frozen and only the output
%   layer is tuned.}
% \label{tab:conll_frz_cased_tst}
% \end{center}
% \end{table}


==> tables/conll_test_cased_perf_by_frz_layers.tex <==

\begin{table}
\begin{center}
\begin{tabular}{lrrr}
\toprule
lang &   deu &   esp &   ned \\
frz &       &       &       \\
\midrule
-1  & 68.99 & 72.83 & 77.18 \\
 0  & 66.42 & 74.61 & 77.33 \\
 1  & 70.21 & 72.63 & 78.58 \\
 2  & 70.41 & 72.76 & 78.58 \\
 3  & 70.63 & 74.99 & 79.50 \\
 4  & 70.37 & 74.24 & 79.37 \\
 5  & 69.72 & 73.42 & 77.58 \\
 6  & 68.71 & 72.63 & 77.81 \\
 7  & 67.30 & 73.44 & 77.53 \\
 8  & 63.97 & 72.58 & 76.28 \\
 9  & 57.62 & 71.30 & 73.58 \\
 10 & 41.96 & 66.09 & 71.07 \\
 11 & 47.00 & 64.42 & 69.55 \\
 12 & 33.56 & 49.82 & 48.89 \\
\bottomrule
\end{tabular}

\caption{}
\label{tab:conll_test_cased_perf_by_frz_layers}
\end{center}
\end{table}


==> tables/conll_test_cased_perf_by_frz_layers_mli.tex <==

\begin{table}
\begin{center}
\begin{tabular}{llrrr}
\toprule
   & lang &   deu &   esp &   ned \\
model & frz &       &       &       \\
\midrule
LI & -1  & 66.52 & 70.15 & 71.85 \\
   &  6  & 65.25 & 68.08 & 74.97 \\
   &  8  & 66.19 & 72.48 & 75.40 \\
ML & -1  & 68.99 & 72.83 & 77.18 \\
   &  0  & 66.42 & 74.61 & 77.33 \\
   &  1  & 70.21 & 72.63 & 78.58 \\
   &  2  & 70.41 & 72.76 & 78.58 \\
   &  3  & 70.63 & 74.99 & 79.50 \\
   &  4  & 70.37 & 74.24 & 79.37 \\
   &  5  & 69.72 & 73.42 & 77.58 \\
   &  6  & 68.71 & 72.63 & 77.81 \\
   &  7  & 67.30 & 73.44 & 77.53 \\
   &  8  & 63.97 & 72.58 & 76.28 \\
   &  9  & 57.62 & 71.30 & 73.58 \\
   &  10 & 41.96 & 66.09 & 71.07 \\
   &  11 & 47.00 & 64.42 & 69.55 \\
   &  12 & 33.56 & 49.82 & 48.89 \\
\bottomrule
\end{tabular}

\caption{}
\label{tab:conll_test_cased_perf_by_frz_layers_mli}
\end{center}
\end{table}


==> tables/ontonotes_ext_exps_cased_dev.tex <==
\begin{table}
\begin{center}
\begin{tabular}{llrrr}
\toprule
      & lang &   arb &   chn &   eng \\
model & frz &       &       &       \\
\midrule
CL & -1 & 18.80 & 82.99 & 82.15 \\
      &  8 & 16.46 & 83.71 & 77.64 \\
CL+LI & -1 &   nan & 82.43 & 81.40 \\
      &  8 & 12.81 & 81.62 & 74.72 \\
LI & -1 &  2.35 & 80.50 & 78.59 \\
      &  8 &  4.19 & 88.89 & 75.56 \\
PC & -1 & 18.98 & 81.98 & 79.07 \\
      &  8 & 15.29 & 83.32 & 77.99 \\
PC+LI & -1 &   nan & 87.50 & 79.36 \\
      &  8 & 14.46 & 84.25 & 74.88 \\
\bottomrule
\end{tabular}
\caption{Ontonotes dev results using LI, CL, CL+LI and different
  frozen layers.}
\label{tab:ontonotes_ext_exps_cased_dev}
\end{center}
\end{table}


==> tables/ontonotes_ext_exps_cased_tst.tex <==

\begin{table}
\begin{center}
\begin{tabular}{llrrr}
\toprule
      & lang &  arb &   chn &   eng \\
model & frz &      &       &       \\
\midrule
CL & -1  & 4.10 & 53.28 & 62.20 \\
      &  8  & 4.63 & 53.89 & 57.52 \\
CL+LI & -1  &  nan & 52.59 & 60.42 \\
      &  8  & 3.68 & 48.79 & 57.58 \\
LI & -1  & 0.23 & 57.12 & 59.33 \\
      &  8  & 0.61 & 61.05 & 55.15 \\
ML & -1  & 3.78 & 53.34 & 60.96 \\
      &  0  & 4.39 & 56.25 & 62.02 \\
      &  1  & 3.79 & 58.35 & 62.02 \\
      &  2  & 5.60 & 61.52 & 62.60 \\
      &  3  & 6.47 & 62.30 & 62.13 \\
      &  4  & 3.55 & 62.06 & 61.98 \\
      &  5  & 6.19 & 64.10 & 60.86 \\
      &  6  & 5.68 & 63.48 & 60.77 \\
      &  7  & 4.49 & 60.48 & 59.08 \\
      &  8  & 5.13 & 59.91 & 58.03 \\
      &  9  & 2.07 & 55.42 & 52.81 \\
      &  10 & 3.10 & 50.70 & 49.04 \\
      &  11 & 5.64 & 50.48 & 45.10 \\
      &  12 & 1.92 & 43.82 & 26.23 \\
PC & -1  & 3.83 & 55.58 & 62.90 \\
      &  8  & 5.35 & 56.13 & 59.27 \\
PC+LI & -1  &  nan & 52.93 & 63.28 \\
      &  8  & 4.16 & 57.92 & 57.26 \\
\bottomrule
\end{tabular}
\caption{Ontonotes test results using ML, LI, CL, CL+LI and different
  frozen layers.}
\label{tab:ontonotes_ext_exps_cased_tst}
\end{center}
\end{table}


==> tables/ontonotes_ext_exps_cased_tst2.tex <==
\begin{table}
\begin{center}
\begin{tabular}{llrrr}
\toprule
      & lang &   arb &   chn &   eng \\
model & frz &       &       &       \\
\midrule
CL & -1 & 15.00 & 85.61 & 79.75 \\
      &  8 & 20.83 & 86.05 & 76.29 \\
CL+LI & -1 &   nan & 84.27 & 79.30 \\
      &  8 & 18.28 & 83.83 & 74.37 \\
LI & -1 &  0.73 & 84.26 & 76.14 \\
      &  8 &  0.54 & 84.33 & 74.96 \\
PC & -1 & 18.76 & 86.45 & 77.79 \\
      &  8 & 13.23 & 86.83 & 76.03 \\
PC+LI & -1 &   nan & 77.92 & 79.11 \\
      &  8 & 13.33 & 88.64 & 74.31 \\
\bottomrule
\end{tabular}
\caption{Ontonotes test results using LI, CL, CL+LI and different
  frozen layers.}
\label{tab:ontonotes_ext_exps_cased_tst2}
\end{center}
\end{table}


==> tables/table_all.tex <==
\begin{figure*}[t]
  \begin{center}
    \begin{tabular}{l|l|rrr|rrr}
      \toprule
          {} & {}       & \multicolumn{3}{c|}{dev} & \multicolumn{3}{c}{test} \\
          \cline{3-8}
          {} & {}       & P     & R     & F     & P     & R     & F     \\
          \midrule
          \multirow{7}{*}{Dutch} &
               baseline & 77.11 & 78.29 & 77.69 & 71.79 & 73.31 & 72.54 \\ \cline{2-8}
             & LI       & 80.30 & 74.66 & 77.38 & 74.62 & 70.95 & 72.74 \\
             & LI+WL    & 40.36 & 75.80 & 52.68 & 34.07 & 71.68 & 46.19 \\
             & CL       & 80.04 & 77.71 & 78.86 & 74.18 & 74.45 & 74.32 \\
             & CL+LI    & 75.02 & 79.78 & 77.32 & 71.16 & 75.74 & 73.38 \\
             & PC       & 77.69 & 77.75 & 77.72 & 76.00 & 74.09 & 75.04 \\
             & PC+LI    & 76.00 & 78.82 & 77.39 & 72.62 & 74.90 & 73.74 \\
          \midrule
          \multirow{7}{*}{English} &
               baseline & 70.00 & 75.48 & 72.64 & 67.06 & 73.74 & 70.24 \\ \cline{2-8}
             & LI       & 70.85 & 73.91 & 72.35 & 65.09 & 68.98 & 66.98 \\
             & LI+WL    & 65.68 & 69.67 & 67.62 & 63.08 & 66.94 & 64.95 \\
             & CL       & 73.02 & 78.54 & 75.68 & 68.63 & 75.64 & 71.96 \\
             & CL+LI    & 74.90 & 80.81 & 77.75 & 71.03 & 78.10 & 74.40 \\
             & PC       & 73.57 & 79.43 & 76.39 & 69.68 & 76.72 & 73.03 \\
             & PC+LI    & 75.83 & 75.93 & 75.88 & 72.71 & 74.24 & 73.46 \\
          \midrule
          \multirow{7}{*}{German} &
               baseline & 84.25 & 81.48 & 82.84 & 76.48 & 75.50 & 75.98 \\ \cline{2-8}
             & LI       & 82.29 & 81.94 & 82.12 & 74.57 & 75.44 & 75.00 \\
             & LI+WL    & 72.53 & 77.96 & 75.15 & 63.39 & 73.45 & 68.05 \\
             & CL       & 82.88 & 83.32 & 83.10 & 74.93 & 76.83 & 75.87 \\
             & CL+LI    & 83.01 & 83.72 & 83.36 & 75.57 & 76.80 & 76.18 \\
             & PC       & 80.98 & 83.34 & 82.15 & 73.16 & 76.97 & 75.02 \\
             & PC+LI    & 82.20 & 80.84 & 81.51 & 73.77 & 74.65 & 74.21 \\
          \midrule
          \multirow{7}{*}{Spanish} &
               baseline & 67.43 & 71.51 & 69.41 & 67.26 & 69.32 & 68.27 \\ \cline{2-8}
             & LI       & 65.61 & 68.77 & 67.15 & 65.55 & 66.93 & 66.23 \\
             & LI+WL    & 62.08 & 63.19 & 62.63 & 64.28 & 63.56 & 63.92 \\
             & CL       & 67.26 & 75.23 & 71.02 & 66.59 & 72.69 & 69.51 \\
             & CL+LI    & 63.62 & 75.18 & 68.92 & 63.17 & 73.93 & 68.13 \\
             & PC       & 61.46 & 70.22 & 65.55 & 62.20 & 70.10 & 65.92 \\
             & PC+LI    & 65.05 & 72.40 & 68.53 & 65.00 & 70.97 & 67.86 \\
          \bottomrule
    \end{tabular}
    \caption{Overall results. The target language of interest is indicated on the far left. Each experimental condition/model is tabulated per row. LI is language identification. WL is pairwise weighted loss. CL is the Cloze task. PC is the predictive Cloze task. +LI indicates that a language ID task has also been added to the objective.}
    \label{tab:all}
  \end{center}
\end{figure*}

==> tables/table_de_es.tex <==
\begin{table*}[t]
  \begin{center}
    \begin{tabular}{l|l|rrr|rrr}
      \toprule
          {} & {}       & \multicolumn{3}{c|}{dev} & \multicolumn{3}{c}{test} \\
          \cline{3-8}
          {} & {}       & P     & R     & F     & P     & R     & F     \\
          \midrule
          \multirow{7}{*}{German} &
               baseline & 84.25 & 81.48 & 82.84 & 76.48 & 75.50 & 75.98 \\ \cline{2-8}
             & LI       & 82.29 & 81.94 & 82.12 & 74.57 & 75.44 & 75.00 \\
             & LI+WL    & 72.53 & 77.96 & 75.15 & 63.39 & 73.45 & 68.05 \\
             & CL       & 82.88 & 83.32 & 83.10 & 74.93 & 76.83 & 75.87 \\
             & CL+LI    & 83.01 & 83.72 & \textbf{83.36} & 75.57 & 76.80 & \textbf{76.18} \\
             & PC       & 80.98 & 83.34 & 82.15 & 73.16 & 76.97 & 75.02 \\
             & PC+LI    & 82.20 & 80.84 & 81.51 & 73.77 & 74.65 & 74.21 \\
          \midrule
          \multirow{7}{*}{Spanish} &
               baseline & 67.43 & 71.51 & 69.41 & 67.26 & 69.32 & 68.27 \\ \cline{2-8}
             & LI       & 65.61 & 68.77 & 67.15 & 65.55 & 66.93 & 66.23 \\
             & LI+WL    & 62.08 & 63.19 & 62.63 & 64.28 & 63.56 & 63.92 \\
             & CL       & 67.26 & 75.23 & \textbf{71.02} & 66.59 & 72.69 & \textbf{69.51} \\
             & CL+LI    & 63.62 & 75.18 & 68.92 & 63.17 & 73.93 & 68.13 \\
             & PC       & 61.46 & 70.22 & 65.55 & 62.20 & 70.10 & 65.92 \\
             & PC+LI    & 65.05 & 72.40 & 68.53 & 65.00 & 70.97 & 67.86 \\
          \bottomrule
    \end{tabular}
    \caption{Results for German and Spanish. The target language of interest is indicated on the far left. Each experimental condition/model is tabulated per row. LI is language identification. WL is pairwise weighted loss. CL is the Cloze task. PC is the predictive Cloze task. +LI indicates that a language ID task has also been added to the objective. The best F-score per setting, language and test set is highlighted in bold.}
    \label{tab:de-es}
  \end{center}
\end{table*}

==> tables/table_du_en.tex <==
\begin{table*}[t]
  \begin{center}
    \begin{tabular}{l|l|rrr|rrr}
      \toprule
          {} & {}       & \multicolumn{3}{c|}{dev} & \multicolumn{3}{c}{test} \\
          \cline{3-8}
          {} & {}       & P     & R     & F     & P     & R     & F     \\
          \midrule
          \multirow{7}{*}{Dutch} &
               baseline & 77.11 & 78.29 & 77.69 & 71.79 & 73.31 & 72.54 \\ \cline{2-8}
             & LI       & 80.30 & 74.66 & 77.38 & 74.62 & 70.95 & 72.74 \\
             & LI+WL    & 40.36 & 75.80 & 52.68 & 34.07 & 71.68 & 46.19 \\
             & CL       & 80.04 & 77.71 & \textbf{78.86} & 74.18 & 74.45 & 74.32 \\
             & CL+LI    & 75.02 & 79.78 & 77.32 & 71.16 & 75.74 & 73.38 \\
             & PC       & 77.69 & 77.75 & 77.72 & 76.00 & 74.09 & \textbf{75.04} \\
             & PC+LI    & 76.00 & 78.82 & 77.39 & 72.62 & 74.90 & 73.74 \\
          \midrule
          \multirow{7}{*}{English} &
               baseline & 70.00 & 75.48 & 72.64 & 67.06 & 73.74 & 70.24 \\ \cline{2-8}
             & LI       & 70.85 & 73.91 & 72.35 & 65.09 & 68.98 & 66.98 \\
             & LI+WL    & 65.68 & 69.67 & 67.62 & 63.08 & 66.94 & 64.95 \\
             & CL       & 73.02 & 78.54 & 75.68 & 68.63 & 75.64 & 71.96 \\
             & CL+LI    & 74.90 & 80.81 & \textbf{77.75} & 71.03 & 78.10 & \textbf{74.40} \\
             & PC       & 73.57 & 79.43 & 76.39 & 69.68 & 76.72 & 73.03 \\
             & PC+LI    & 75.83 & 75.93 & 75.88 & 72.71 & 74.24 & 73.46 \\
          \bottomrule
    \end{tabular}
    \caption{Results for Dutch and English. The target language of interest is indicated on the far left. Each experimental condition/model is tabulated per row. LI is language identification. WL is pairwise weighted loss. CL is the Cloze task. PC is the predictive Cloze task. +LI indicates that a language ID task has also been added to the objective. The best F-score per setting, language and test set is highlighted in bold.}
    \label{tab:du-en}
  \end{center}
\end{table*}

==> tables/table_multitrain_orig.tex <==
\makeatletter
\setlength{\@fptop}{0pt}
\makeatother

\begin{table*}[ht!]\label{table1}

\begin{tabular}{|l|c|c|c|c|}
\hline 
{\small{}{System}} & {\small{}{English}} & {\small{}{Spanish}} & {\small{}{German}} & {\small{}{Dutch}}\tabularnewline
\hline 
{\small{}CoNLL'02 and '03} & {\small{}{88.6}} & {\small{}{81.4}} & {\small{}{72.4}} & {\small{}{77.1}}\tabularnewline
\hline 
{\small{}\citet{Baevski19-cloze5}} & {\small{}\textbf{93.5}} & {\small{}{-}} & {\small{}{-}} & {\small{}{-}}\tabularnewline
\hline 
{\small{}\citet{akbik-etal-2018-contextual}} & {\small{}{93.2}} & {\small{}{-}} & {\small{}\textbf{88.2}} & {\small{}{90.4}}\tabularnewline
\hline 
{\small{}\citet{BERT18}} & {\small{}{92.6}} & {\small{}{-}} & {\small{}{-}} & {\small{}{-}}\tabularnewline
\hline 
{\small{}\citet{LampleBSKD16}} & {\small{}{90.9}} & {\small{}{85.8}} & {\small{}{78.8}} & {\small{}{81.7}}\tabularnewline
\hline 
{\small{}Flair-ML} & {\small{}{92.2}} & {\small{}{86.6}} & {\small{}{74.9}} & {\small{}{88.9}}\tabularnewline
\hline \hline
{\small{}{BERT-SL (this work)}} & {\small{}{91.2}} & {\small{}87.5} & {\small{}82.7} & {\small{}{90.6}}\tabularnewline
\hline 
{\small{}{BERT-ML (this work)}} & {\small{}{91.3}} & {\small{}\textbf{87.9}} & {\small{}{83.3}} & {\small{}\textbf{91.1}} \tabularnewline
\hline 
\end{tabular}{\small{}{\small{}\vspace*{2mm}}}%
\begin{tabular}{|p{2.8cm}|c|c|c|}
\hline 
{\small{}{System}} & {\small{}{English}} & {\small{}{Arabic}} & {\small{}{Chinese}}\tabularnewline
\hline 
{\small{}{\cite{akbik-etal-2018-contextual}}} & {\small{}\textbf{89.7}} & {\small{}{-}} & {\small{}{-}}\tabularnewline
\hline 
{\small{}{\cite{clark-etal-2018-semi}}} & {\small{}{88.8}} & {\small{}{-}} & {\small{}{-}}\tabularnewline
\hline 
{\small{}{\cite{ghaddar-langlais-2018-robust}}} & {\small{}{88.0}} & {\small{}{-}} & -\tabularnewline
\hline 
{\small{}{\cite{pradhan-etal-2013-towards}}}\vspace*{0.48cm} & {\small{}82.4} & {\small{}{68.0}} & {\small{}{71.8}}\tabularnewline
\hline \hline
{\small{}{BERT-SL (this work)}} & {\small{}{87.9}} & {\small{}{68.7}} & {\small{}{72.9}}\tabularnewline
\hline 
{\small{}{BERT-ML (this work)}} & {\small{}{88.3}} & {\small{}\textbf{69.9}} & {\small{}\textbf{74.1}}\tabularnewline
\hline 
\end{tabular}{\small\par}

{\small{}\caption{Single and multi language F$_{1}$ on CoNLL'02, CoNLL'03 (left) and OntoNotes (right). Flair-ML is the system described in \cite{akbik-etal-2018-contextual}, trained multilingually, available from \cite{akbik19:flair}\label{table:Multitrain}.}
}{\small\par}
\end{table*}


==> tables/table_ontonotes_ext_exps.tex <==
\begin{table*}[t]
  \begin{center}
\begin{tabular}{llrrrrrr}
\toprule
                    & test\_data &  arabic.development.ner.iob1 &  arabic.test.ner.iob1 &  chinese.development.ner.iob1 &  chinese.test.ner.iob1 &  english.development.ner.iob1 &  english.test.ner.iob1 \\
task\_name & bert\_freeze\_layer\_size &                              &                       &                               &                        &                               &                        \\
\midrule
ZSMentionTask\_CL & -1 &                    18.803419 &             23.463687 &                     82.985658 &              85.612648 &                     82.152169 &              80.468750 \\
                    &  8 &                    16.455696 &             20.833333 &                     83.705650 &              86.365422 &                     77.638564 &              76.291861 \\
ZSMentionTask\_CL\_LI & -1 &                          NaN &                   NaN &                     82.429784 &              84.269663 &                     81.402660 &              79.921741 \\
                    &  8 &                    12.811388 &             18.282548 &                     81.621801 &              83.825944 &                     74.715972 &              74.820144 \\
ZSMentionTask\_LI & -1 &                     2.352941 &              1.465201 &                     80.499836 &              84.257386 &                     78.586878 &              78.236265 \\
                    &  8 &                     4.186795 &              3.521127 &                     88.888889 &              87.408013 &                     75.556516 &              75.187287 \\
ZSMentionTask\_PC & -1 &                    18.983051 &             18.764302 &                     81.979030 &              86.451613 &                     79.067577 &              79.233382 \\
                    &  8 &                    15.286624 &             18.253968 &                     83.322884 &              86.846405 &                     77.992614 &              76.031215 \\
ZSMentionTask\_PC\_LI & -1 &                          NaN &                   NaN &                     87.500000 &              82.527881 &                     79.360320 &              79.159623 \\
                    &  8 &                    14.457831 &             19.246862 &                     84.251969 &              88.640000 &                     74.881087 &              74.305556 \\
\bottomrule
\end{tabular}
\caption{Overall results. The target language of interest is indicated
  on the far left. Each experimental condition/model is tabulated per
  row. LI is language identification. WL is pairwise weighted loss. CL
  is the Cloze task. PC is the predictive Cloze task. +LI indicates
  that a language ID task has also been added to the objective.}
\label{tab:all}
\end{center}
\end{table*}


==> tables/table_zershot_old.tex <==
\begin{table*}[ht!]
{\small{}}%
\begin{tabular}{|p{2.7cm}|c|c|c|c|}
\hline 
{\small{}{System}} & {\small{}{English}} & {\small{}{{Spanish}}} & {\small{}{{German}}} & {\small{}{{Dutch}}}\tabularnewline
\hline 
{\small{}{\citet{Xie2018}}} & {\small{}-} & {\small{}{}72.4} & {\small{}{}56.9} & {\small{}{}71.3}\tabularnewline
\hline 
{\small{}{BERT-SL$^{Eng}$} 0-shot} & {\small{}{91.2}} & {\small{}{75.1}} & {\small{}{74.6}} & {\small{}{78.3}}\tabularnewline
\hline 
{\small{}{BERT-ML$^3$ 0-shot}} & {\small{}{}71.5} & {\small{{}{76.4}}} & {\small{69.9}} & {\small{}{80.6}}\tabularnewline
\hline 
{\small{}{\ \ \ +50 HoL Sents}} & {\small{}{-}} & {\small{}{-}} & {\small{}{72.9}} & {\small{}{82.0}}\tabularnewline
\hline 
{\small{}{\ \ \ +100 HoL Sents}} & {\small{}{-}} & {\small{}{-}} & {\small{}{74.7}} & {\small{}{82.1}}\tabularnewline
\hline 
{\small{}{\ \ \ +200 HoL Sents}} & {\small{}{-}} & {\small{}{-}} & {\small{}{75.0}} & {\small{}{83.2}}\tabularnewline
\hline 
{\small{}WordPiece fertility} & {\small{}{}1.93}  & \small{} {{}2.11}& {\small{}{2.55}} & {\small{}{{}2.38}}\tabularnewline
\hline 
\end{tabular}{\small{} }%
\begin{tabular}{|p{2.8cm}|c|c|c|}
\hline 
{\small{}{System}} & {\small{}{English}} &  {\small{}{{Arabic}}}&{\small{}{{Chinese}}} \tabularnewline
\hline
- & - & - & - \tabularnewline
\hline
{\small{}{BERT-SL$^{Eng}$ 0-shot}} & {\small{}{87.9}}&{\small{}{10.7}} &{\small{}65.2} \tabularnewline
\hline
{\small{}{BERT-ML$^2$ 0-shot}} & {\small{}61.0} &  {\small{}12.6}& {\small{}65.6} \tabularnewline
\hline 
{\small{}{\ \ \ +50 HoL Sents}} & {\small{}{-}}  & {\small{}33.4}& {\small{}66.9}\tabularnewline
\hline 
{\small{}{\ \ \ +100 HoL Sents}} & {\small{}{-}}  & \small{} {42.1}& {\small{}{67.3}} \tabularnewline
\hline 
{\small{}{\ \ \ +200 HoL Sents}} & {\small{}{-}}  & \small{} {47.6}& {\small{}{68.4}}\tabularnewline
\hline 
{\small{}{WordPiece fertility}} & {\small{}{1.8}}  & \small{}{7.42}& {\small{}{2.31}}\tabularnewline
\hline 
\end{tabular}{\small\par}

{\small{}\caption{Zero-shot/Low-resource F$_{1}$ scores for models trained on three
CoNLL (left)/two OntoNotes languages (right) and tested on the held-out-language (HoL). BERT-ML$^k$ is the BERT-ML system trained on $k$ languages.\label{table:zeroshot}}
}{\small\par}
%\vspace*{-14mm}
\end{table*}



